Dolphins: Multimodal Language Model for Driving

The quest for fully autonomous vehicles (AVs) capable of navigating complex real-world scenarios with human-like understanding and responsiveness. In this paper, we introduce Dolphins, a novel vision-language model architected to imbibe human-like abilities as a conversational driving assistant. Dolphins is adept at processing multimodal inputs comprising video (or image) data, text instructions, and historical control signals to generate informed outputs corresponding to the provided instructions. Building upon the open-sourced pretrained Vision-Language Model, OpenFlamingo, we first enhance Dolphins's reasoning capabilities through an innovative Grounded Chain of Thought (GCoT) process. Then we tailored Dolphins to the driving domain by constructing driving-specific instruction data and conducting instruction tuning. Through the utilization of the BDD-X dataset, we designed and consolidated four distinct AV tasks into Dolphins to foster a holistic understanding of intricate driving scenarios. As a result, the distinctive features of Dolphins are characterized into two dimensions: (1) the ability to provide a comprehensive understanding of complex and long-tailed open-world driving scenarios and solve a spectrum of AV tasks, and (2) the emergence of human-like capabilities including gradient-free instant adaptation via in-context learning and error recovery via reflection.

==> subtex/limitations.tex <==
\section{Limitation}

In this section, we summarize the limitations of \model{} as follows:

\begin{enumerate}[leftmargin=*]
\item \textbf{Evaluation.} We show some demonstrations from three views, including perception, prediction, and planning on both zero- and few-shot settings. There is a survey~\cite{li2023multimodal} highlighting the existence of more than 10 diverse multimodal benchmarks. However, assessing the capabilities of VLMs effectively remains unexplored. Consequently, we are still in the process of investigating an efficient and comprehensive evaluation method for \model{} in terms of multiple tasks in ADS.
\item \textbf{Autonomous Driving-Related Task Diversity.} Although examples shown by us demonstrate \model's robust comprehension of a wide array of instructions, we acknowledge that the emergence of these abilities relies on the visual instructions fine-tuned foundation model~\cite{anonymous2023understanding}. To further enhance the applicability of \model{} in ADs, it is imperative to construct a more diverse dataset of instructions encompassing tasks such as perception, detection, tracking, reasoning, prediction, and planning.
\item \textbf{Various Multimodal Features in ADS.} The first version of \model{} involves only inputting the model with video data captured by the front camera, which is acknowledged to have limitations. Therefore, in our future endeavors, we plan to incorporate additional multimodal features such as Bird's Eye View~(BEV), road maps, and point cloud features to develop a more comprehensive end-to-end autonomous driving system built upon VLMs.
\end{enumerate}

We acknowledge these limitations and are working to address them in our future work.
